Directed Regular and Context-Free Languages

We study the problem of deciding whether a given language is directed. A language $L$ is \emph{directed} if every pair of words in $L$ have a common (scattered) superword in $L$. Deciding directedness is a fundamental problem in connection with ideal decompositions of downward closed sets. Another motivation is that deciding whether two \emph{directed} context-free languages have the same downward closures can be decided in polynomial time, whereas for general context-free languages, this problem is known to be coNEXP-complete. We show that the directedness problem for regular languages, given as NFAs, belongs to $AC^1$, and thus polynomial time. Moreover, it is NL-complete for fixed alphabet sizes. Furthermore, we show that for context-free languages, the directedness problem is PSPACE-complete.

==> sections/main-technique-regular.tex <==
% !TEX root = ../main.tex
Now we have an ideal decomposition of $\dcl{L(\NFA)}$ given via $L(\NFAidl)$. 
It is well-known that every ideal contained in a finite union of downward closed sets, is contained in exactly one of those downward closed sets. That is,
\begin{lemma}\label{lemma:dwclosedunion}\ISinside{Citation to be found.}
If $I$ is an ideal and $I \subseteq \bigcup_{i \in [1, m]} D_i$ for some $m \in \N$ and downward closed sets $D_i$, then $I \subseteq D_j$ for one $j \in [1,m]$. 
\end{lemma}
%\begin{claimproof}
%    The proof follows by induction. For the base case let $m = 1$. Then the claim trivially holds. Now assume the claim holds for $m = k-1$ and show that is holds for $m = k$.
%If $I$ is contained in $(k-1)$-many $D_i$, then the claim holds by the induction step. If not, then for all $j \in [1,m]$ there exists a distinct element $d_j \in D_j \setminus \bigcup_{i \in [1,k] \setminus \{j\}} D_i$ such that $d_j \in I$ for all $j \in [1,m]$.
%Since $I$ is upward directed it contains an element $y \succeq d_1, \ldots, d_k$.
%This $y$ cannot belong to any of the downward closed sets, since otherwise the downward closed set that contains $y$ would contain all $d_1, \ldots, d_k$. This contradiction gives $I \subseteq D_j$ for one $j \in [1,k]$.
%\end{claimproof}

Observe that if $\dcl{L(\NFA)}$ is upward directed, it is, by definition, an ideal. 
Since $\dcl{L(\NFA)}$ is contained in the union of the ideals $\NFAidl$ accepts~\eqref{eq:Lidealdecomp}, %(note that all ideals in $L(\NFAidl)$ are downward closed sets), 
if it is upward directed, by~\cref{lemma:dwclosedunion} it is equal to one of the ideals in $L(\NFAidl)$.

We naturally want to check if such an ideal exists, since the answer will give us the answer to the directedness of $\dcl{L(A)}$.
That's why, we want to obtain `the biggest' ideal in $L(\NFAidl)$. 

Such a quest requests us to have some kind of a measure on ideal representations, that will allow us to compare ideal representations and conclude which one is `bigger'.
In the next section, we introduce the tools that allow us this comparison. 

\subsection{Tools for comparing ideal representations}

We want to have a measure on ideal representations that satisfies two properties: \begin{inparaenum}\item the summation of the measures of atoms in the representation give the measure of the ideal representation, and\label{inpara:item1} \item for ideals $I$ and $J$ represented by $A_1 \ldots A_n$ and $B_1 \ldots B_m$, respectively; if $I \subseteq J$, the measure of $I$ is larger than that of $J$. Furthermore if $I\neq J$, the inequality is strict.\label{inpara:item2}\end{inparaenum}

In this subsection, we will first introduce the weight function that satisfies~\cref{inpara:item1}, then introduce an embedding on ideals. Via this embedding we will prove that the weight function satisfies~\cref{inpara:item2} for reduced representations, in Theorem \ref{prop:weightfunc}. 

In this subsection, we will first introduce the weight function that satisfies~\cref{inpara:item1}, then introduce an embedding on ideals. Via this embedding we will prove that the weight function satisfies~\cref{inpara:item2} for reduced representations, in Theorem \ref{prop:weightfunc}. 
From there on, we will use this weight function as a measure with desired properties on reduced ideal representations. 
\subsubsection{The weight function}\label{subsec:weight-function}

For a given $k \in \N$, the ($k$-)weight of an ideal representation $A_1 \ldots A_n$ is defined as,
 $\mu_k(A_1 \ldots A_n) = \sum^{n}_{i=1} \mu_k(A_i)$ where
\begin{align}\label{eq:idealweight}
     \mu_k(A_i) = \begin{cases}
        1, &\text{ if } \,\, A_i \text{ is a single atom }\\
        (k+1)^{|\Delta|}, &\text{ if } \,\, A_i = \atomt \text{ for some } \emptyset \neq \Delta \subseteq \Sigma.     \end{cases}
\end{align}
%$\mu_k(A_1\ldots A_n)$ is called the \emph{$k$-weight} of $A_1\ldots A_n$.
$\mu_k(\cdot)$ satisfies~\cref{inpara:item1} by construction. 
In fact, we cannot have a `smaller' weight function that satisfies~\cref{inpara:item2}. To see this, look at the exponential-length chain $C_k$ of ideals over the alphabet $\Sigma = \{x_1, \ldots, x_k\}$ constructed as follows:
For $i \in [1, k]$, let $\Sigma_i$ represent the set $\{x_1, \ldots, x_i\}$. Set $C_0 := (\Atomi{x_1})$.
 For each $i \in [1, k]$, assuming $C_{i-1} = (I_1, \ldots, I_t)$, set $C_i$ as
$$C_{i} := (I_1, \ldots, I_t, \Atomt{(\Sigma_{i-1})}\cdot\Atomi{x_t}\cdot I_1,  \ldots,  \Atomt{(\Sigma_{i-1})}\cdot \Atomi{x_t} \cdot I_t)$$
Clearly, the length of $C_k$ is exponential in $k$. Moreover, each ideal in $C_k$ has polynomial length w.r.t. $k$. 
The chain is strict since for each $i$, $x_i$ does not appear in $C_{i-1}$. 
Therefore, the desired weight function maps each ideal in $C_k$ to a distinct value.
\IS{should I have mentioned that we cannot have an NL algorithm here?}

On the other hand, $\mu_k(\cdot)$ does not satisfy~\cref{inpara:item2} on arbitrary ideal representations. For instance, consider the ideals represented by $\Atomt{a}\cdot\Atomt{a}$ and $\Atomt{a}\cdot\Atomt{b}$. 
The latter contains the former, but they have the exact same weight. 
In~\cref{prop:weightfunc} we show that $\mu_k(\cdot)$ satisfies~\cref{inpara:item2} on reduced ideal representations. 
To show this, we need the following embedding function.

\subsubsection{The embedding function}

\begin{restatable}{lemma}{restatableembedding}\label{lemma:embedding}
    Let $A_1\cdots A_n$ and $B_1 \cdots B_m$ be representations of ideals $I$ and $J$ on $\Sigma$, respectively. If $I \subseteq J$, then there exists a function $f : [1, n] \to [1, m]$ such that 
    \begin{enumerate}
        \item $f(i)\leq f(i+1)$ for all $i\in [1, n-1]$,  \label{line:one}
        \item $A_i$ is contained in $B_{f(i)}$ for all $i \in [1,n]$, \label{line:two}
        \item if $B_j$ is a single atom, then $|f^{-1}(B_j)|\leq 1$ \label{line:three}
      %  \item if $f(i) = j$ and $B_j$ is a single atom, then $A_i$ is also a single atom.\ISinside{is this necessary?}
    \end{enumerate}
\end{restatable}
\begin{proof}[Proof sketch] For each atom $A$, we generate a unique word $\wordatom{A}$. If the atom is $\atomi$, then the word $\wordatom{A} = a$. 
If the atom is an alphabet atom $A = \atomt$, then we fix an order on $\Sigma$ and for each $\Delta \subseteq \Sigma$ let $\worddelta{\Delta}$ be some word that contains each letter in $\Delta$ once, in the increasing order.
Then the word $\wordatom{A} = \worddelta{\Delta}^{m+1}$. 
We define the embedding function $f:[1, n] \to [1,m]$ such that, 
$f$ sends each $i$ to the $j$ for which $B_1 \ldots B_j$ is the shortest prefix of $B_1 \ldots B_m$ for which $\wordatom{A_1} \ldots \wordatom{A_i} \in \Idl(B_1 \ldots B_j)$. It is easy to verify that this $f$ satisfies the premises of~\cref{line:one}-\ref{line:three}.
\end{proof}


We use the embedding function $f$ to show $\mu_k(\cdot)$ satisfies~\cref{inpara:item2}.
\begin{proposition}\label{prop:weightfunc}
Let $A_1\cdots A_n$ and $B_1 \cdots B_m$ be reduced ideal representations of the non-empty ideals $I$ and $J$, respectively. For any $k \geq \max\{n,m\}$, if $I \subseteq J$ then $\mu_k(A_1 \cdots A_n) \leq \mu_k(B_1 \cdots B_m)$. 
Moreover, if $I \subsetneq J$, then $\mu_k(A_1 \cdots A_n) < \mu_k(B_1 \cdots B_m)$. 
\end{proposition}
\begin{proof}
 For the given ideal representations $A_1 \cdots A_n$ and $B_1 \cdots B_m$ let $f: [1,n]\to [1,m]$ be the embedding function introduced in~\cref{lemma:embedding}.
    \begin{claim*}
    For all $j \in [1,m]$, $\quad\mu_k(B_j) \geq \sum_{i\in f^{-1}(j)} \mu_k(A_i)$
    \end{claim*}
    \begin{claimproof}[Proof of claim]
        If $B_j$ is a single atom, then by~\cref{line:three}, there exists at most one $A_i$ embedded to $B_j$. Furthermore by~\cref{line:two}, $B_j$ contains $A_i$. By the definition of containment, we get that $A_i$ is a single atom (and in fact, is identical with $B_j$). In this case, $\mu_k(B_j) = \mu_k(A_i) = 1$.
        Otherwise, $B_j = \atomt$. By~\cref{line:one}, the elements of $f^{-1}(j)$ have to be consecutive numbers. That is, the set $f^{-1}(j)$ is an interval $[i_1, i_2]$. Then $A_{i_1}, A_{{i_1}+1}, \dots, A_{i_2}$ are the atoms embedded in $B_j$ by $f$. Since the representation $A_1\ldots A_n$ is reduced, each $A_i$, $A_{i+1}$ pair is non-absorptive. Since they are all contained in $B_j$, either $|f^{-1}(j)|=1$, or for all $i \in [i_1, i_2]$, $|A_i| < |B_j|$ where $|A_i| = 0$ if $A_i$ is a single atom; otherwise it is the size of the alphabet of $A_i$. This is because otherwise one $A_i$ would have to be equal to $B_j$, and thus would contain all $A_{i_1}\ldots A_{i_2}$ and $f^{-1}(j)$ would have size one. 
        In the first case where $|f^{-1}(j)| = 1$, since the only atom in $f^{-1}(j)$ is contained in $B_j$, the claim trivially holds. In the latter case, the following inequality follows from
        the fact that $f$ can embed at most $n$ many atoms into $B_j$ and that $n \leq k$, 
        \begin{equation}\label{eq:weightsupset}
            \sum_{i\in f^{-1}(j)} \mu_k(A_i) \leq n\cdot {(k+1)}^{|\Delta|-1} < (k+1)^{|\Delta|} = \mu_k(B_j). 
        \end{equation}    
    \end{claimproof}

    Since the weight of an ideal representation is defined as the sum of the weights of its atoms, and $f$ embeds each atom of $A_1\ldots A_n$ into an atom of $B_1\ldots B_m$, it follows from the claim that $\mu_k(B_1\ldots B_m) \geq \mu_k(A_1\ldots A_n)$. This concludes the first part of the proof.

    Now assume $I \subsetneq J$.  Thus, either there exists $i \in [1,n]$ such that $A_i$ is strictly contained in $B_j$,
    or $f$ is not surjective. In the latter case, 
    \begin{equation}\label{eq:strictineq}
    \mu_k(A_1\ldots A_n) < \mu_k(B_1 \ldots B_m)
    \end{equation}
     follows from the previous argument. In the former case, $B_j$ must be an alphabet atom, otherwise it cannot strictly contain an $A_i$. 
    If $A_i$ is a single atom, then the weight of $A_i$ is $1$, and equation~\ref{eq:strictineq} holds. 
    If $A_i$ is also an alphabet atom, then equation~\ref{eq:strictineq} follows from formula~\ref{eq:weightsupset}.
\end{proof}
%\MG{It would be good if you could avoid ``by construction'' arguments so that the reader can basically
%forget the proof of the previous theorem and just work with its statement.}\IS{Done for the proof above.}

==> sections/old-solution-regular.tex <==

\subsection{Old Solution on Regular $L$}
Let $L$ be a regular language and $ \mathbf{A}=(Q, \Sigma, \delta, q_0, F)$ an NFA with a unique initial state $q_0$ and without unreachable states, that recognizes $L$. %We can find the strongly connected components of $\mathbf{A}$ in linear time using Kosaraju's algorithm. 
We can calculate the strongly connected components of $\mathbf{A}$ in $\NL$ by the following procedure:
We define a linear order on $Q$, and check for each node $v_i \in Q$ whether there exists a $v_j\in Q$ with $v_j < v_i$ and $v_i$ and $v_j$ are mutually reachable. This procedure gives a negative answer for a $v_i$ if and only if $v_i$ is the smallest node in its SCC. Representing all the SCCs via their smallest nodes, we can list the SCCs explicitly.
Since reacability is in $\NL$ and we only need to store two pointers for $v_i$ and $v_j$, this procedure is in $\NL$.  

Now let $\{S_1, \ldots S_n\}$ where $S_i\subseteq Q$ be the set of connected components of $\mathbf{A}$. Next we construct an $\emp-$NFA by collapsing the connected components similar to the construction of a condensation graph.
\begin{equation*}
    \mathcal{A}_{SCC} = (\hat{Q} = \{s_1, \dots, s_n\},\Sigma, \hat{\delta}, \hat{q_0}, \hat{F} ) \text{ where }
\end{equation*}

%\MG{$\log {|Q| \choose k} \approx k \log |Q|$ which is not log-space if $k$ is not constant.
%Here's how you can compute the SCCs of a digraph: Define some linear order on the nodes.
%Compute for each SCC the smallest node, by going through each node $v$ one by one,
%and test that there is no smaller node reachable from $v$.
%Now, having a representative for each SCC, you can list the SCCs.} \IS{Done for the proof above.}

\begin{itemize}
    \item $\hat{\delta}(s_i, a) = s_j$ and iff there exists a $q_i \in S_i$  and  $q_j \in S_j$ with $\delta(q_i, a) = q_j$,
    \item $\hat{q_0} = s_i$ for the $i$, $q_0 \in S_i$,
    \item $s_i\in \hat{F}$ if and only if $F\cap S_i \neq \emptyset$.
\end{itemize}

Observe that the only cycles $\mathcal{A}_{SCC}$ contains are self-loops.

\begin{theorem}
    If $L$ is downward closed, then $L(\mathcal{A}_{SCC}) = L$.
\end{theorem}

\begin{proof}
    $\mathbf{(L\subseteq L(\mathcal{A}_{SCC}))}$ This side is easy to see. Let $q_0 \xrightarrow{a_1} q_1 \xrightarrow{a_2} \dots q_{n-1} \xrightarrow{a_{n}} q_f$ be an accepted path of $\mathbf{A}$ and $\mathbf{a} = a_1\dots a_n$ the corresponding accepted word. Since all transitions are still existent in $\mathcal{A}_{SCC}$ and $q_{n-1} \xrightarrow{a_n} q_f$ corresponds to a transition $s_{k} \xrightarrow{a_n} s_f$ in $\mathcal{A}_{SCC}$ where $s_f \in \hat{F}$, $\mathbf{a}\in L(\mathcal{A}_{SCC})$.

    $\mathbf{(L(\mathcal{A}_{SCC})\subseteq L)}$. Let $s_0 \xrightarrow{a_1} s_1 \xrightarrow{a_2} \dots s_{n-1} \xrightarrow{a_{n}} s_f$ be an accepted path of $\mathcal{A}_{SCC}$ for some $s_f \in \hat{F}$ and $\mathbf{a} = a_1\dots a_n$ the corresponding accepted word. $s_i \xrightarrow{a_{i+1}} s_{i+1}$ implies that there is a transition $q \xrightarrow{a_{i+1}} q'$ for some $q\in S_i$ and $q' \in S_{i+1}$. Since $S_i$s are SCCs, it follows that, for any $\mathbf{q_i} \in S_i$ and $\mathbf{q_{i+1}} \in S_{i+1}$, there exists a path $\mathbf{q_i} \xrightarrow{w a_{i+1}w'} \mathbf{q_{i+1}}$ for some $w, w' \in \Sigma^*$. This implies that there is a path $q_0 \xrightarrow{w_1 a_1 w_2 \dots a_n w_{n+1}} q_f$ for some $q_f\in S_f$.  Since $L$ is downward closed, this gives $\mathbf{a} \in L$.
\end{proof}
From this point on, we will take $L=\dcl{L}$.
Since the only cycles $\mathcal{A}_{SCC}$ contains are self-loops, we can write $L$ as a finite union of all accepted paths of $\mathcal{A}_{SCC}$ as follows,
\begin{equation*}
    L = L(\mathcal{A}_{SCC}) = \bigcup_{i \in \{1,\ldots,r\}} a_{1,i} \Delta_{1,i}^* a_{2,i} \Delta_{2,i}^* \ldots a_{k_i,i} \Delta_{k_i,i}^*
\end{equation*}
where all $a_{n,i} \in \Sigma \cup \{\emp\}$ and all $\Delta_{n,i}\subseteq \Sigma$.
Since $L$ is downward closed, we can represent $L(\mathcal{A}_{SCC})$ further as
\begin{equation*}
    L = L(\mathcal{A}_{SCC}) = \bigcup_{i \in \{1,\ldots, r\}} \{\emp, a_{1,i}\} \Delta_{1,i}^* \{\emp, a_{2,i}\} \Delta_{2,i}^* \ldots \{\emp,a_{k_i,i}\} \Delta_{k_i,i}^*
\end{equation*}
which is exactly a finite union of ideals on $\Sigma$. However, these ideal representations do not have to be in normal form.

Next, we will construct a new NFA $\mathcal{A}^{flat}$ on the alphabet of atoms of $\Sigma$.

Let $Atoms(\Sigma)$ be the set of all atoms on $\Sigma$. % Note that the size of $Atoms(\Sigma)$ is exponential in the size of $\Sigma$.
$\mathcal{A}^{flat} = (Q^\mathfrak{f}, Atoms(\Sigma), \lambda^{\mathfrak{f}}, q^\mathfrak{f}_0, F^{\mathfrak{f}})$ is constructed as follows, 
\begin{itemize}
    \item For each state $q \in \hat{Q}$, for which there exists a $\hat{\delta}(q,a) = q$ for some $a \in \Sigma$,
    \begin{itemize}
        \item define a new state $\bar{q}$ and add $q, \bar{q} \in Q^\mathfrak{f}$,
        \item define $\lambda^\mathfrak{f}(q,\Delta^*) = \bar{q}$ where $\Delta = \{a\in \Sigma \mid \hat{\delta}(q, a) = q\}$,
        \item for all $q\neq p \in \hat{Q}$ with $\hat{\delta}(q, \emp) = p$, define $\lambda^\mathfrak{f}(\bar{q},\emp) = p$,
        \item for all $q\neq p \in \hat{Q}$ with $\hat{\delta}(q, a) = p$ for some $a \in \Sigma$, define $\lambda^\mathfrak{f}(\bar{q},\{a, \emp\}) = p$,
        \item whenever $q \in \hat{F}$, let $\bar{q} \in F^\mathfrak{f}$.
    \end{itemize}
    \item For each state $q \in \hat{Q}$, for which there exists no $\hat{\delta}(q,a) = q$ for some $a \in \Sigma$,
    \begin{itemize}
        \item add $q \in Q^\mathfrak{f}$,
        \item for all $q\neq p \in \hat{Q}$ with $\hat{\delta}(q, \emp) = p$, define $\lambda^\mathfrak{f}(q,\emp) = p$,
        \item for all $q\neq p \in \hat{Q}$ with $\hat{\delta}(q, a) = p$ for some $a \in \Sigma$, define $\lambda^\mathfrak{f}(q,\{a, \emp\}) = p$,
        \item whenever $q \in \hat{F}$, let $q \in F^\mathfrak{f}$.
    \end{itemize}
    \item Let $q^\mathfrak{f}_0 = \hat{q_0}$.
\end{itemize}

Observe that $\mathcal{A}^{flat}$ is an acyclic $\emp-$NFA where $|Q^{\mathfrak{f}}| \leq 2\cdot |\hat{Q}| \leq 2 \cdot |Q|$, $\,|\lambda^{\mathfrak{f}}| \leq |\hat{\delta}| \leq |\delta|$, $\,|F^\mathfrak{f}| = |\hat{F}| \leq |F|$ and $|Atoms(\Sigma)| = 2^{|\Sigma|}$. It is easy to see that given $A^{SCC}$, $\mathcal{A}^{flat}$ can be constructed in logarithmic space. 

Also note that, between two states $p, q \in Q^{\mathfrak{f}}$, there is either one transition of an alphabet atom $p \xrightarrow{\Delta^*} q$, an $\emp-$transition or $i-$many transitions of single atoms $p \xrightarrow{\{\emp, b_i\}} q$ where $1 \leq i \leq |\Sigma|$. Thus, $|\lambda^{\mathfrak{f}}| \leq 2\cdot|\hat{Q}|\cdot |\Sigma| \leq 2\cdot|Q|\cdot |\Sigma| $.

\begin{notation}
    With slight abuse of notation, for a letter $u \in Atoms(\Sigma)$ and a word $w \in \Sigma^*$, we write $w \in u$ if $w$ is in the language represented by the atom $u$. Similarly, for a sequence of atoms $u_1\ldots u_k$, we write $w \in u_1\ldots u_k$ if there exists a decomposition $w = v_1\ldots v_k$ of $w$ for some $v_i \subseteq \Sigma^*$ where for all $i \in \{1, \ldots, k\}$, $v_i \in u_i$. 
\end{notation}
\begin{definition}
    A word $w \in \Sigma^*$ is called \textbf{internally-accepted} by an atom-labeled NFA $A$ on $Atoms(\Sigma)$ if there exists an accepted word $I \in L(A)$ such that $w \in I$.
   %A word $w = v_1 \ldots v_k$ where all $v_i \in \Sigma^*$ is called \textbf{internally-accepted} by an atom-labeled NFA $A$ on $Atoms(\Sigma)$ if there exists an accepted word $I = u_1\ldots u_k \in L(A)$ such that $v_i \in u_i$ for all $i\in \{1, \ldots, k\}$.
   %A word $w = v_1 \ldots v_l$ on $\Sigma'$ is called \textbf{internally-accepted} by an atom-labeled NFA $A$ if there exists an accepted word $I = u_1\ldots u_k \in L(A)$, where each $u_i \in Atoms(\Sigma')$ and a function $f_{w, I}:\{1, \ldots, l\} \to \{1, \ldots k \}$ that satisfies the following,
   % \begin{itemize}\label{itemize:embedfunc}
   %     \item For all $i \in \{1, \ldots, l-1\}$, $ f_{w,I}(i) \leq f_{w,I}(i+1)$, 
   %     \item If $f_{w,I}(i) = j$, then $v_i \in u_j$.
   % \end{itemize}
   % Requiring the existence of such a function $f_{w,I}$, is equivalent to requiring $w$ to be in the language of the ideal represented by $I$.
    
    The words internally-accepted by $A$ is said to constitute its internal language, $IL(A)$.
\end{definition}

The words that are internally-accepted by $\mathcal{A}^{flat}$ are exactly the words accepted by $\mathcal{A}_{SCC}$, that is, $IL(\mathcal{A}^{flat}) = L$.
In this sense, the accepted words of $\mathcal{A}^{flat}$ represent a set $S$ of ideals of $L$, for which $\bigcup S = L$.

Next, we want to construct an $\emp-$NFA $\mathcal{A}^{norm}$ for which $IL(\mathcal{A}^{norm}) = IL(\mathcal{A}^{flat}) = L$ and all the words in $L(\mathcal{A}^{norm})$ are normal representations of some ideals. 
 
$\mathcal{A}^{norm}$ is defined as a tuple $ (Q^{\mathfrak{n}}, E^{\mathfrak{n}}, l^{\mathfrak{n}}, q^{\mathfrak{n}}_0, F^{\mathfrak{n}})$ where
\begin{itemize}
    \item $Q^{\mathfrak{n}}$ is the finite state set,
    \item $E^{\mathfrak{n}} \subseteq Q^{\mathfrak{n}} \times Q^{\mathfrak{n}}$ is the unlabeled transition relation between states,
    \item $l^{\mathfrak{n}}: Q^{\mathfrak{n}} \to Atoms(\Sigma) \cup \{\emp\}$ is the labeling function on states, 
    \item $q^{\mathfrak{n}}_0 \in Q^{\mathfrak{n}}$ is the initial state,
    \item $F^{\mathfrak{n}} \subseteq Q^{\mathfrak{n}}$ is the set of final states
\end{itemize}
\IS{The next paragraph is probably unnecessary:}
A path $q_0 q_1 \ldots q_k$ of $\mathcal{A}^{norm}$ is called accepted if $q_0 = q^{\mathfrak{n}}_0$, $q_k \in F^{\mathfrak{n}}$ and for each $i \in \{0, \ldots, k-1\}$, $(q_i, q_{i+1}) \in E^{\mathfrak{n}}$. A word $w \in Atoms(\Sigma) \cup \{\emp\}$ is said to be accepted by $\mathcal{A}^{norm}$ if and only if there exists an accepted path $q_0 \ldots q_k$ with $l(q_0)\ldots l(q_k) = w$.
The set of all word accepted by $\mathcal{A}^{norm}$ is said to be the language of it and denoted by $L(\mathcal{A}^{norm})$.
The internal language of $\mathcal{A}^{norm}$ is defined similarly.
We set,
\begin{itemize}
    \item $Q^{\mathfrak{n}} = \{\mathbf{q}_{q_i, a_i, q_j} \mid \lambda^{\mathfrak{f}}(q_i, a_i) = q_j\} \cup \{q_0^{\mathfrak{n}}\}$
    \item For all $\mathbf{q}_{q_i, a_i, q_j}, \mathbf{q}_{q'_i, a'_i, q'_j} \in Q^{\mathfrak{n}}$, $(\mathbf{q}_{q_i, a_i, q_j}, \mathbf{q}_{q'_i, a'_i, q'_j}) \in E^{\mathfrak{n}}$ if there exists a path from $q_j $ to $q'_i$ in $\mathcal{A}^{flat}$ and $a_i$ and $a'_i$ are incomparable, or one of them is $\emp$,
    \item For all $\mathbf{q}_{q_i, a_i, q_j} \in Q^{\mathfrak{n}} $ where $q_i$ is reachable from $q_0^{\mathfrak{f}}$ in $\mathcal{A}^{norm}$, $(q_0^{\mathfrak{n}}, \mathbf{q}_{q_i, a_i, q_j}) \in E^{\mathfrak{n}}$, 
    \item For all $\mathbf{q}_{q_i, a_i, q_j} \in Q^{\mathfrak{n}} $ where a state $q \in F^{\mathfrak{f}}$ is reachable from $q_j$ in $\mathcal{A}^{flat}$, $(\mathbf{q}_{q_i, a_i, q_j}, q_f^{\mathfrak{n}}) \in E^{\mathfrak{n}}$, 
    \item For all $\mathbf{q}_{q_i, a_i, q_j} \in Q^{\mathfrak{n}}$, $l( \mathbf{q}_{q_i, a_i, q_j}) = a_i$ and $l(q_f^{\mathfrak{n}}) = l(q_0^{\mathfrak{n}}) = \emp$,
    \item For all  $\mathbf{q}_{q_i, a_i, q_j} \in Q^{\mathfrak{n}} $ where $q_j \in F^{\mathfrak{f}}$, $\mathbf{q}_{q_i, a_i, q_j} \in F^{\mathfrak{n}}$
\end{itemize}
Note that $\mathcal{A}^{norm}$ is acyclic, since there is a path between two states $\mathbf{q}_{q_i, a_i, q_j}, \mathbf{q}_{q'_i, a'_i, q'_j}$ of $\mathcal{A}^{norm}$ only if there is a path between $q_i$ and $q'_i$ in $\mathcal{A}^{flat}$, and $\mathcal{A}^{flat}$ is acyclic.
\begin{proposition}
    $ IL(\mathcal{A}^{norm}) = IL(\mathcal{A}^{flat})$
 \end{proposition}
 \begin{proof}
 $\mathbf{(IL(\mathcal{A}^{norm}) \subseteq IL(\mathcal{A}^{flat})})$
 Take an $I = l(\mathbf{q}_0^{\mathfrak{n}}) l(\mathbf{q}_{q_1, a_1, p_1})\ldots l(\mathbf{q}_{q_k, a_k, p_k}) \in L(\mathcal{A}^{norm})$. 
 $\mathbf{q}_0^{\mathfrak{n}} \mathbf{q}_{q_1, a_1, p_1}\ldots \mathbf{q}_{q_k, a_k, p_k}$ is an accepted path. That is, $(\mathbf{q}_0^{\mathfrak{n}},\mathbf{q}_{q_1, a_1, p_1}) \in E^{\mathfrak{n}}$, $\mathbf{q}_{q_k, a_k, p_k} \in F^{\mathfrak{n}}$ and $(\mathbf{q}_{q_i, a_i, p_i}, \mathbf{q}_{q_{i+1}, a_{i+1}, p_{i+1}}) \in E^{\mathfrak{n}}$ for each $i\in \{1, \ldots, k-1\}$. Then, for each such $i$, there exists a path from $q_i$ to $q_{i+1}$ in $\mathcal{A}^{flat}$ with $q_i \xrightarrow{a_i\ldots} q_{i+1}$, where $q_1$ is the initial state and $p_k$ is a final state of $\mathcal{A}^{flat}$ . 
 It follows that there exists an accepted path $q_0^{\mathfrak{f}} \xrightarrow{a_1\ldots} q_2 \xrightarrow{a_2 \ldots} \ldots \xrightarrow{a_{k-1}\ldots} q_k \xrightarrow{a_k} p_k$ of $\mathcal{A}^{flat}$. Since $L$ is downward closed, for any word $w \in I$, there exists a word $J \in L(\mathcal{A}^{flat})$ with $I \preccurlyeq J$. Naturally, $w \in J$. This argument concludes the first side of the proof.


 \par $\mathbf{( IL(\mathcal{A}^{norm}) \supseteq IL(\mathcal{A}^{flat}))}$
     Let $w= u_1\ldots u_l \in IL(\mathcal{A}^{flat})$. 
     Let $\hat{q_0} q_1 \ldots q_k$ be the accepted path of $\mathcal{A}^{flat}$ on which $w$ is read, that is $\hat{q_0} \xrightarrow{u_1} q_1 \xrightarrow{u_2} q_2 \xrightarrow{u_3} \ldots \xrightarrow{u_{k-1}} q_{k-1} \xrightarrow{u_k} q_k$ for $q_k \in F^{\mathfrak{f}}$. 
     Let $u'_1 \ldots u'_{k'}$ be a subword of $u_1 \ldots u_k$ where each $u'_i, u'_{i+1}$ are incomparable. By the construction of $E^{\mathfrak{n}}$, all such subwords are accepted by $\mathcal{A}^{norm}$. In other words, all subwords of $u_1 \ldots u_k$ that are normal representations of some ideals, are in $L(\mathcal{A}^{norm})$. 
     Theorem \ref{thm:existsnormalform} proves that for every ideal $I$, there exists an ideal $J$ that is in its normal form with $L(I) = L(J)$. An inspection of the induction in the proof of the theorem reveals that additionally, there exists such a $J$ with $J \preccurlyeq I$. Thus, for all $I \in L(\mathcal{A}^{flat})$, there exists a $J \in L(\mathcal{A}^{norm})$ such that $J \preccurlyeq I$ with $L(I) = L(J)$.
     It follows that, for any word $w \in I$ for some $I \in L(\mathcal{A}^{flat})$, there exists a $J \in L(\mathcal{A}^{norm})$ with $J \preccurlyeq I$ and thus, $w \in J$.
     This concludes the proof by showing that if $w \in IL(\mathcal{A}^{flat})$, then $w \in IL(\mathcal{A}^{norm})$.
 \end{proof}

Finally, we argue that given $\mathcal{A}^{flat}$, we can compute $\mathcal{A}^{norm}$ in $\NL$. 

We can encode each state $\mathbf{q}_{q_i, a_i, q_j}$ using $O(log(|\lambda^{\mathfrak{f}}|)) = O(log(|Q|\cdot|\Sigma|))$ space. For each $\mathbf{q}_{q_i, a_i, q_j} \neq \mathbf{q}_{q'_i, a'_i, q'_j} \in Q^{\mathfrak{n}}$, we guess that there is a path between $q_j$ and $q'_i$ in $\mathcal{A}^{flat}$ and calculate whether $a_i$ and $a'_i$ are comparable in $O(log(|\Sigma|))$ space. If they are comparable, we write down the edge $(\mathbf{q}_{q_i, a_i, q_j}, \mathbf{q}_{q'_i, a'_i, q'_j})$ to $E^{\mathfrak{n}}$. Since $l^{\mathfrak{n}}$ and $F^{\mathfrak{n}}$ can also be calculated in logarithmic space, the overall procedure is completed in non-deterministic $O(log(|Q|\cdot|\Sigma|))$ space. 
\IS{Even lower?}

Next, we construct a weight-labeled $\emp-$NFA $\mathcal{A}^\mu = (Q^{\mathfrak{n}}, E^{\mathfrak{n}}, l^{\mu}, q^{\mathfrak{n}}_0, F^{\mathfrak{n}})$ out of $\mathcal{A}^{norm}$ by solely changing the labeling function. (\IS{Perhaps we do not need to define a new NFA, it is sufficient to define the new labeling}) $l^\mu: Q^{\mathfrak{n}} \to \mathbb{N}$ where for each $\mathbf{q} \in Q^{\mathfrak{n}}$, $l^\mu(\mathbf{q}) = \mu_{\enn}(l^{\mathfrak{n}}(\mathbf{q}))$. If $l^{\mathfrak{n}}(\mathbf{q}) = \emp$, we assign $l^{\mu}(\mathbf{q}) = 0$. Let $\enn = |Q^\mathfrak{n}|$, then $\enn$ is an upper bound on the length of any ideal of $L$; thus, by theorem~\ref{prop:weightfunc}, for any $I, J \subseteq L$,  $I \subseteq J \implies \mu_{\enn}(I) \leq \mu_{\enn}(J)$.

If $L$ is upward directed, then it is an ideal itself. By theorem \ref{prop:weightfunc}, for all ideals $I$ of $L$, $\mu_{\enn}(L) \geq \mu_{\enn}(I)$. Since $L = \bigcup \{I \mid I \in L(\mathcal{A}^{norm})\}$, all ideals in $L$ are subwords of some $I \in L(\mathcal{A}^{norm})$. Thus, an ideal $I \in L(\mathcal{A}^{norm})$ satisfying $\mu_{\enn}(I) = max\{ \mu_\enn(J) \mid J \in L(\mathcal{A}^{norm})\}$, should be equal to $L$. 
Note that if there are multiple such $I$, then all of them should be equal to $L$.

For some $I \in L(\mathcal{A}^{norm})$ accepted by the path $\mathbf{q}_0 \mathbf{q}_1 \ldots \mathbf{q}_k$, $\mu_{\enn}(I) = \sum_{0 \leq i \leq k} l(\mathbf{q}_i)$.
To calculate the accepted path of $\mathcal{A}^{\mu}$ with the maximum weight, we have to sum up the labels of its states. To do so, we put an order on the states of $Q^{\mathfrak{n}}$ and construct an $\enn \times \enn$-matrix $\mathcal{M}$, the elements of which takes values from the \textit{max-plus semiring}, which is the semiring $(\mathbb{R}\cup \{-\infty\},\otimes, \oplus)$ with operations 
\begin{align*}
 &x \otimes y := x+y\\
 &x \oplus y := max\{x,y\}
\end{align*}
where the unity of $\oplus$ is $-\infty$ and the unity of $\otimes$ is 0. Then for each $i,j \leq \enn$,
\begin{align*}
\mathcal{M}(i,j) = \begin{cases}
 l^{\mu}(\mathbf{q}_i) &\text{ if } (\mathbf{q}_i, \mathbf{q}_j) \in E^{\mathfrak{n}}\\
 -\infty  &\text{ if } (\mathbf{q}_i, \mathbf{q}_j) \not \in E^{\mathfrak{n}}
\end{cases}
\end{align*}
Without loss of generality, assume $\mathbf{q}_f^{\mathfrak{n}} = \mathbf{q}_{\enn}$ and $\mathbf{q}_0^{\mathfrak{n}} = \mathbf{q}_1$. Assigning $\mathcal{M}(\enn, \enn) = 0$ gives us an $\emp-$self loop on the unique final state.
Multiplying (on the semiring operations) $\mathcal{M}$ with itself for $\enn$ times, we get $\mathcal{M}^{\enn}$. $\mathcal{M}^{\enn}(1, \enn)$ gives us the maximum weight of an accepted path in $\mathcal{A}^\mu$. \IS{I think I will need to prove this}
Raising a matrix to its $\enn$th power can be done in $\AC^1$ \IS{citation}. Say the maximum weight obtained is $\mathfrak{w}_{max}$. Then in $\NL$, we can find a path of $\mathcal{A}^\mu$ with weight $\mathfrak{w}_{max}$ by guessing.

Once we have 'a' maximum weight accepted path $\mathbf{q}_1\ldots\mathbf{q}_k$, we check whether the ideal $I_{max} = l^\mathfrak{n}(\mathbf{q}_1)\ldots l^{\mathfrak{n}}(\mathbf{q}_k)$ contains $L$. Checking whether $\dcl{M} \subseteq \dcl{N}$ for a language $M$ given by an NFA, and an ideal $N$ is $\NL$-complete \cite{icalpZetzsche16}.
So, in the general case, the complexity of the overall procedure is determined by the matrix multiplication, which is in $\AC^1$, since all other translations can be completed by $\NL$ transductions. 

In the case of a fixed alphabet, the matrix multiplication is not needed and the whole procedure is in $\NL$. 

If $\Sigma$ is fixed, we do not have to calculate the maximum weight path, instead we can store all the potential weights a path in $\mathcal{A}^\mu$ can get, and try them one by one, starting from to maximum possible weight. The main idea is as follows, we set the number $k = (n+1)^{|\Sigma|}$, which is the maximum weight an ideal contained in $L \subseteq \Sigma^*$ can get (and store $k$ in $O(log(n))$ space). Then we guess that there is an accepted path in $\mathcal{A}^\mu$ with weight $k$ and guess the path. If there is no path with weight $k$, we get to learn it in $\NL$ as well, since $\NL=\coNL$. In this case, we decrement $k$ by $1$ and repeat the process. This way, we go over all the weights an ideal of $L$ can have and we are guaranteed to find a path with the maximum weight. However, more than one path with the maximum weight can exist. In this case, the $\NL$ transduction is not guaranteed the provide a consistent 'maximal path finding' procedure. That's why we need to apply a small trick that allows the path finding algorithm to favor some states over others, and thus produce the same maximum weight path consistently.
We fix an order on the state set $Q^{\mathfrak{n}}$. This order can be determined with respect to the initial NFA $\mathbf{A} = (Q, \Sigma, \delta, q_0, F)$. For $\mathbf{q}_{q_i, a_i, q_j}, \mathbf{p}_{p_i, b_i, p_j} \in Q^{\mathfrak{n}}$, we give higher precedence to $\mathbf{q}_{q_i, a_i, q_j}$ if and only if the transition corresponding to $\hat{\delta}(q_i, a_i) = q_j$ appears first at the input tape. \IS{will elaborate more on this because, $\hat{\delta}$ is actually not in the initial automaton}. 
So, for a fixed weight $k$, whenever the algorithm guesses the successor state $q_{i+1}$ from a state $q_i$ such that the weight of a path $q_1 \ldots q_i q_{i+1}\ldots q_t $ is equal to $k$, it also guesses that $q_{i+1}$ is the state with the highest precedence amongst those in $\{ q_j\in Q^\mathfrak{n} \mid (q_i, q_j)\in E^{\mathfrak{n}} \text{ and } q_1\ldots q_{i} q_j \text{ is the prefix of an accepted path with weight } k\}$.

From a certificate-based approach, the linear size certificate of 'the' accepted path $q_1 \ldots q_t$ provided to the algorithm for a fixed $k$ is accepted if and only if this path both has the weight $k$, and for each $i$; $q_{i+1}$ is the state that has the highest precedence amongst the states in $\{ q_j\in Q^\mathfrak{n} \mid (q_i, q_j)\in E^{\mathfrak{n}} \text{ and } q_1\ldots q_{i} q_j$ is the prefix of an accepted path with weight $k\}$. %So, every time the maximal path finding algorithm runs and guesses the next state for a $q \in Q^\mathfrak{n}$ that gives out the maximal path, 
With the application of this trick, we can find an ideal $I$ of $L$ in its normal form with the maximum weight in $\NL$.

Given an NFA representing the downward closed language $L$, we can decide whether $L$ is upward directed in $\AC^1$; whereas on a fixed alphabet we can decide the same in $\NL$.

%The trick is as follows, we mutliply all weights with the number of states in $\mathcal{A}^\mu$, and assign a unique number $i < \enn$ to each state, and sum up the weight of each state with the number assigned to it. This way, we guarantee that for paths $u, v$, if the weight of $u$ was strictly less than that of $v$, then this procedure preserves the order. If $u$ and $v$ had the same weight, this procedure increases the weight of one, more than the other. So, after this procedure, there exists no two paths with the same weight.

%We endow $\mathcal{A}^{\mu}$ with a new labeling function $\ell: Q^{\mathfrak{n}} \to \enn\cdot (n+1)^{|\Sigma|}+1$. Let $o: Q^{\mathfrak{n}} \to \enn$ be a 1-to-1 function that assigns a unique positive integer to each state. Then $\ell(q) = l^\mu(q)\cdot \enn + o(q)$.
%\begin{proposition} For any two distinct accepted paths $\mathbf{u}, \mathbf{v}$ of $\mathcal{A}^\mu$,
%    \begin{enumerate}
%        \item $\ell(\mathbf{u}) \neq \ell(\mathbf{v})$,
%        \item If $l^\mu(\mathbf{u}) < l^\mu(\mathbf{v})$, then $\ell(\mathbf{u}) < \ell(\mathbf{v})$.
%    \end{enumerate}
%\end{proposition}
